On-demand electrical control of spin qubits

Once called a "classically non-describable two-valuedness" by Pauli , the electron spin is a natural resource for long-lived quantum information since it is mostly impervious to electric fluctuations and can be replicated in large arrays using silicon quantum dots, which offer high-fidelity control. Paradoxically, one of the most convenient control strategies is the integration of nanoscale magnets to artificially enhance the coupling between spins and electric field, which in turn hampers the spin's noise immunity and adds architectural complexity. Here we demonstrate a technique that enables a \emph{switchable} interaction between spins and orbital motion of electrons in silicon quantum dots, without the presence of a micromagnet. The naturally weak effects of the relativistic spin-orbit interaction in silicon are enhanced by more than three orders of magnitude by controlling the energy quantisation of electrons in the nanostructure, enhancing the orbital motion. Fast electrical control is demonstrated in multiple devices and electronic configurations, highlighting the utility of the technique. Using the electrical drive we achieve coherence time $T_{2,{\rm Hahn}}\approx50 \mu$s, fast single-qubit gates with ${T_{\pi/2}=3}$ ns and gate fidelities of 99.93 % probed by randomised benchmarking. The higher gate speeds and better compatibility with CMOS manufacturing enabled by on-demand electric control improve the prospects for realising scalable silicon quantum processors.

==> Degenerate EDSR Mar 18/extData.tex <==


\makeatletter
\renewcommand{\figurename}{Extended Data Figure}
\makeatother
%\makeatletter
%\renewcommand*{\fnum@figure}{{\normalfont\bfseries \figurename~\thefigure}}
%\renewcommand*{\@caption@fignum@sep}{ $|~$}
%\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
%\makeatother

\renewcommand{\tablename}{Extended Data Table}
\makeatletter
\renewcommand*{\fnum@table}{{\normalfont\bfseries \tablename~\thetable}}
%\renewcommand*{\@caption@fignum@sep}{ $|~$}
%\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\captionsetup[table]{name={Extended Data Table},labelsep=period,justification=raggedright,font=small}
\captionsetup[figure]{name={\bf{Extended Data Fig.}},labelsep=line,justification=raggedright,font=small}
\setcounter{figure}{0}

\setcounter{table}{0}


%\section*{Supplementary Note 1: Experimental details}



%Device A - Rainbow (Pd/ALD) - MV25
%
%Device B - Slater (Pd/ALD) - MV24
%
%Device C - Sunshine (Al) - MV24
%
%Device D - Alder (Al) - MV24
\begin{table*}[ht]
\caption{\textbf{Devices details} \newline
Device A was fabricated on an isotopically enriched silicon-28 substrate (50 ppm residual $^{29}$Si) \cite{becker2010enrichment}.
Devices B, C \& D were fabricated on an epitaxially grown, isotopically purified $^{28}$Si epilayer with a residual $^{29}$Si concentration of 800 ppm \cite{itoh2014isotope}.} % title of Table
\label{table:devices} % is used to refer this table in the text
\centering % used for centering table
\begin{tabular}{c c c c c c c} % centered columns (4 columns)
\hline\hline %inserts double horizontal lines
Device & \begin{tabular}{@{}c@{}} $^{29}$Si \\ concentration \end{tabular} & Gate Materials & Electron Occupancy & \begin{tabular}{@{}c@{}}$B_{0}$-Field \\ (T) \end{tabular}  & \begin{tabular}{@{}c@{}}Microwave Carrier \\ Frequency (GHz) \end{tabular} & Mode of Driving \\ [0.5ex] % inserts table
%heading
\hline % inserts single horizontal line
A & 50 ppm & TiPd & (1,3) \& (3,1) & 0.825  & 22.3  & antenna-based \\ % inserting body of the table
B & 800 ppm & TiPd & (3,1) & 0.55  & 15.4  & antenna-based \\
C & 800 ppm & Al & (1,3) & 0.825  & 22.3  & antenna-based \\
D & 800 ppm & Al & (3,1) & 0.1 - 1.0  & 2.8 - 28  & gate-based\\ [1ex] % [1ex] adds vertical space
\hline \hline %inserts double line
\end{tabular}




\end{table*}

\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 1\textwidth, angle = 0]{ExtData2.pdf}
    \caption{\textbf{Calibration of the microwave excitation amplitude}}
    The microwave signal applied to the CB1 gate of Device D is delivered through a transmission line that is poorly characterised for frequencies above 6 GHz. \textbf{a}, Here the line transmission is calibrated by first measuring the slope of Coulomb oscillations relative to the voltages on the sensor top gate and the CB1 gate,  which gives a relative lever arm of 14.8. Then, in \textbf{b} the width of a single Coulomb peak is measured against the microwave amplitude, scaled from a reference level of 0 dBm from the source. The fitted peak width trend in \textbf{c} gives a maximum amplitude at the CB1 gate of $50 \pm 2$~mV when multiplied by the relative lever arm.
    \label{fig:mw_amp}
\end{figure*}
 
\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 0.85\textwidth, angle = 0]{ExtData3.pdf}
    \caption{\textbf{Obtaining degeneracy on demand via excited state spectroscopy}}
    The protocol for tuning the energy spectrum of a new charge configuration to create a level degeneracy, resulting in a speed-up of the qubit Rabi frequency. The protocol utilises excited state spectroscopy, where a differential square wave excitation is applied to $\Delta V_{\mathrm P} = \Delta V_{\mathrm{P1}} = -\Delta V_{\mathrm{P2}}$, with in-phase charge movements detected using double lock-in down-conversion \cite{yang2011dynamically}. $\Delta V_{\mathrm P}$ is swept across an interdot charge transition to observe changes in the interdot tunnel rate associated with the population of excited states \cite{yang2012orbital}.
    \textbf{a}, Top-view schematic layout of the device gates. \textbf{b}, Schematic potential landscapes for increasing $\Delta V_{\mathrm P}$, progressing from deep in (3,1) to deep in (4,0), where in-between the ground state of the P2 dot crosses the level of multiple states for the 4th electron of the P1 dot. In \textbf{g} the two right-most features are designated as states A and B, representing the ground and 1st excited states of the P1 dot.
    To create a level degeneracy we observe the trend in the separation of states A and B whilst deforming the dots, and tune towards a point of zero separation. In \textbf{g}, $V_{\mathrm{P1}}$, $V_{\mathrm{P2}}$, and $V_{\mathrm{J}}$ are varied and denoted as $V_{\mathrm{P,offset}}$, with the expected potential deformation shown in \textbf{c}. The states A \& B appear to converge for decreasing $V_{\mathrm{P,offset}3}$, so we set $V_{\mathrm{P,offset}} = 1.7~V$ and in \textbf{d} \& \textbf{h} re-tune $V_{\mathrm{J}}$ to achieve desired tunnel rates.
    At the lower J value the excited states can be probed again. In \textbf{e} \& \textbf{i} we further lower $V_{\mathrm{P,offset}}$, and lose the visibility of the excited state due to high tunnel rates. In \textbf{f} \& \textbf{j} we again attempt to re-tune the interdot tunnel rate and again observe the states A \& B, here converging for higher $V_{\mathrm{J}}$, potentially a sign that states A \& B have already crossed. Now we perform a PESOS map near the red triangle where we anticipate a degeneracy, with results shown in \ref{fig:pesos}b in the main text. We note that the first PESOS map we took in the vicinity of the red triangle immediately showed a speed up of the qubit Rabi frequency. 
    %Our initial starting point is at the top of right side of \textbf{c}. The schematic potentials along x and y axes are shown in left and middle respectively. To tune the degeneracy, we start by performing the excited state spectroscopy in by applying a large amplitude detuning square pulse (see main for details) and monitoring the excited state through the increased current. We start from the top of the plot and follow the position of the lowest excited state as we lower (in some case we need to increase) the mean of both plunger gates P1 and P2 and the J-gate simultaneously and sweep the detuning voltage. We see the gap of the lowest excited state and the ground state closing up indicating, we are getting closer to degeneracy which in this case is induced by making the potential of the dot shallower (smaller difference w.r.t confinement barriers). At the bottom of the graph the tunnel rates are getting too fast for the excited state to be observable and we continue in \textbf{b}, where we sweep the detuning and lower down the J gate, to increase the visibility of the excited state. We can see the excited state energy to become even closer to degeneracy as we do this. Once we are satisfied with the visibility we continue to shallow the potential of the system in \textbf{c}. We again reach a state at the lower part of the graph where the we see no excited states due to the fast tunnel rates. From the bottom of the graph we move to \textbf{d}, where we lower the J gate voltage to again to observe the excited state at the bottom. This time the excited state energy is increasing at the bottom of the graph indicating that we have gone past the degeneracy point and the expected speed up of Rabi. To measure that we choose the point indicated by red as the readout/initialization point. We then perform PESOS measurement near the orange dot (near expected degeneracy) to obtain the map seen in Fig. 2(b) in the main text.
    \label{fig:obtain_degeneracy}
\end{figure*}
 
%\section*{Supplementary Note 3: Obtaining degeneracy on demand -- charge configurations, gate density and identification of controllable excitation}

%The first time we came across this degeneracy in device A in (1,3) charge configuration for dot 2 was by accident. To convince ourselves that this was not just one off and that dots in general can be tuned to achieve the degeneracy together with rabi speed up we demonstrate a method to tune this degeneracy from scratch for the other charge configuration (3,1) for dot A. In this section we use the excited state spectroscopy to achieve the degeneracy and the resulting speed up of rabi which is already shown in the main text figure 2. 


%In order to demonstrate how reproducible achieving the degeneracy is we perform an exercise of finding the degeneracy at another charge configuration in device A. In the charge configuration (1,3) in device A we found this degeneracy of the dot 2 by accident. The protocol to tune up the device to the degeneracy point is 


%\section*{Supplementary Note 4: Extracting Rabi frequency from PESOS maps}

%textbf{Incomplete section. Waiting on content from Henry}

%The speed up of the Rabi frequency can be observed in the PESOS maps. To extract a Rabi frequency as a function of gate voltage, we fit the Rabi formula to the line cut of the PESOS map. The fit provides both the Larmor and Rabi frequencies. To get a continuous fitting we use the values from the previous line cut as an initial guess for for the next line. An initial estimate of the Rabi and Larmor frequencies is used for the first line based on the Rabi frequency and the

\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 0.8\textwidth, angle = 0]{ExtData5.pdf}
    \caption{\textbf{Enhanced relaxation rate near level degeneracy}}
    The spin relaxation time $T_1$ measuring across the full target charge configurations for Device A (\textbf{a}) and Device D (\textbf{b}) in $V_{\rm J}$ and $\Delta V_{\rm P}$ gate space. The locations of level crossings are indicated as red dashed lines. This shows an enhanced spin relaxation rate near the point of level degeneracy in the respective systems. Interestingly, there are two visible transitions in Device D, between which the spin relaxation is faster than the background, potentially indicating the population of an alternative ground state.
    \label{fig:T1}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 0.95\textwidth, angle = 0]{ExtData6.pdf}
    \caption{\textbf{Diabatic orbital excitation}}
    \textbf{a}, PESOS map in which the ramp time of the J-gate voltage is 80~ns. The resonance frequency continues on a linear trend, indicating that the orbital state is maintained when crossing the point of degeneracy at $V_{\rm J} = 1.638$~V.
    \textbf{b}, PESOS map in which the J-gate ramp time is increased to $2~{\mu}$s. The resonance frequency jumps after the degeneracy point, indicating population of a new orbital state via adiabatic passage across the level-crossing.
    \label{fig:diabatic}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 0.8\textwidth, angle = 0]{ExtData10.pdf}
    \caption{\textbf{Rabi Frequency Compensation}}
    \textbf{a} and \textbf{b} show Rabi oscillations discretised into ${\pi}/2$ rotations and repeated 10 times to observe instability, with Rabi frequency feedback on, and off, respectively. The feedback protocol measures $P_{\rm flip}$ for 5, 7, 9, and 11 ${\pi}/2$ pulses, each of which should result in a 0.5 flip proportion in the ideal case. It then applies a correction to the microwave amplitude of $\delta A_{\rm MW} = - gain * [P_5 - P_7 + P_9 - P_{11}]$, where $P_n$ is the measured spin flip proportion after $n$ ${\pi}/2$ rotations.
    \label{fig:rabifb}
\end{figure*}

\begin{figure*}[ht!]
    \centering
    %\hspace{-0.6cm}
    \includegraphics[width = 0.8\textwidth, angle = 0]{ExtData11.pdf}
    \caption{\textbf{Comparison of driving gates for EDSR}}
    \textbf{a}, PESOS map acquired with microwave drive applied to the CB1 gate.
    \textbf{b}, A PESOS map acquired using the same configuration as for \autoref{fig:qubit}, with microwave drive applied to the J-gate.
    Both measurements use the same source power of 20 dBm, however variation in line losses due to different electronics may result in differences in electric field amplitude applied to the CB1- and J-gates.
   % \textbf{c} PESOS map acquire with microwave drive applied to the J gate, where the power is reduced to match electric field measured by the SET using the method described in Ext Data \autoref{fig:mw_amp}. We suspect there to be significant variation in measured relative lever arms between measurements at DC and at 22 GHz. 
    \label{fig:drivegate}
\end{figure*}

==> Degenerate EDSR Mar 18/table.tex <==
\vspace{3cm}


%\definecolor{y}{RGB}{195,4,51}
%\definecolor{x}{RGB}{2,136,192}
%\definecolor{y}{RGB}{220,220,220}
%\definecolor{x}{RGB}{220,220,220}
%\definecolor{b}{RGB}{220,220,220}

\definecolor{y}{RGB}{255,255,255}
\definecolor{x}{RGB}{255,255,255}
\definecolor{b}{RGB}{255,255,255}

\begin{table}[t]
    \centering
     \setlength{\tabcolsep}{0pt}
        \caption{Coefficients used to construct $\sqrt{\rm{X}}$ and $\sqrt{\rm{Y}}$ gates with \autoref{eq:xy} for different duration and $\Omega_{\rm{R}}=1\,\text{MHz}$.%\chy{is it 1 MHz or 1.4 MHz? should also include period of 7 since thats the main simulated figures you have}
        }
        \setlength\extrarowheight{2pt}
        \begin{tabular}{cc|cc|c}
        %\toprule
        %\toprule
        \hline
        \hline
        \multicolumn{2}{c|}{$\sqrt{\rm{X}}$} & \multicolumn{2}{c|}{$\sqrt{\rm{Y}}$} &\multicolumn{1}{c}{}  \\
        \hline
        \multicolumn{1}{c}{$\nu^{x}_{v}$ (MHz) $\hspace{0.1cm}$} &\multicolumn{1}{c|}{$\nu^{x}_{w}$ (MHz)$\hspace{0.3cm}$}   &$\hspace{0.3cm}$\multicolumn{1}{c}{$\nu^{y}_{v}$ (MHz) $\hspace{0.1cm}$}  &
        \multicolumn{1}{c|}{$\nu^{y}_{w}$ (MHz) $\hspace{0.1cm}$}
        &\multicolumn{1}{c}{$\hspace{0.3cm}$ $\tau$ ($T_{\rm{mod}})$} \\
        \hline
        0.1515 & 0.3336  & -0.2154& 0.2224  & 1\\
        0.0893 & 0.1579  &-0.1056 &  0.1136 & 2\\
        0.0620 & 0.0921  &-0.0701 &  0.0760 & 3\\
        0.0271 & 0.0366  &-0.0300 & 0.0327  & 7\\
        0.0190 & 0.0254  &-0.0210 &  0.0229 & 10\\
        %\bottomrule
        %\bottomrule
        \hline
        \hline
    \end{tabular}
    \label{tab:tab}
\end{table}




==> table.tex <==
\vspace{3cm}


%\definecolor{y}{RGB}{195,4,51}
%\definecolor{x}{RGB}{2,136,192}
%\definecolor{y}{RGB}{220,220,220}
%\definecolor{x}{RGB}{220,220,220}
%\definecolor{b}{RGB}{220,220,220}

\definecolor{y}{RGB}{255,255,255}
\definecolor{x}{RGB}{255,255,255}
\definecolor{b}{RGB}{255,255,255}

\begin{table}[t]
    \centering
     \setlength{\tabcolsep}{0pt}
        \caption{Coefficients used to construct $\sqrt{\rm{X}}$ and $\sqrt{\rm{Y}}$ gates with \autoref{eq:xy} for different duration and $\Omega_{\rm{R}}=1\,\text{MHz}$.%\chy{is it 1 MHz or 1.4 MHz? should also include period of 7 since thats the main simulated figures you have}
        }
        \setlength\extrarowheight{2pt}
        \begin{tabular}{cc|cc|c}
        %\toprule
        %\toprule
        \hline
        \hline
        \multicolumn{2}{c|}{$\sqrt{\rm{X}}$} & \multicolumn{2}{c|}{$\sqrt{\rm{Y}}$} &\multicolumn{1}{c}{}  \\
        \hline
        \multicolumn{1}{c}{$\nu^{x}_{v}$ (MHz) $\hspace{0.1cm}$} &\multicolumn{1}{c|}{$\nu^{x}_{w}$ (MHz)$\hspace{0.3cm}$}   &$\hspace{0.3cm}$\multicolumn{1}{c}{$\nu^{y}_{v}$ (MHz) $\hspace{0.1cm}$}  &
        \multicolumn{1}{c|}{$\nu^{y}_{w}$ (MHz) $\hspace{0.1cm}$}
        &\multicolumn{1}{c}{$\hspace{0.3cm}$ $\tau$ ($T_{\rm{mod}})$} \\
        \hline
        0.1515 & 0.3336  & -0.2154& 0.2224  & 1\\
        0.0893 & 0.1579  &-0.1056 &  0.1136 & 2\\
        0.0620 & 0.0921  &-0.0701 &  0.0760 & 3\\
        0.0271 & 0.0366  &-0.0300 & 0.0327  & 7\\
        0.0190 & 0.0254  &-0.0210 &  0.0229 & 10\\
        %\bottomrule
        %\bottomrule
        \hline
        \hline
    \end{tabular}
    \label{tab:tab}
\end{table}



